Search for the decay $B^- \rightarrow \Lambda_c^+ \bar{p} \ell^- \bar{\nu}_{\ell}$ with the BABAR detector

This work presents the search for the semileptonic baryonic B decay $B^- \rightarrow \Lambda_c^+ \bar{p} \ell^- \bar{\nu}_{\ell}$. The used data comprises the complete BABAR data set of $470 \cdot 10^{6}$ $B\bar{B}$ events, collected at the SLAC National Accelerator Laboratory. Using a pole-model decay simulation, we obtain upper limits with $90\%$ confidence level of $B(B^- \rightarrow \Lambda_c^+ \bar{p} e^- \bar{\nu}_{e})\cdot \frac{B(\Lambda_c^+ \rightarrow p K^- \pi^+)}{5\%} < 1.2 \times 10^{-4}$, $B(B^- \rightarrow \Lambda_c^+ \bar{p} \mu^- \bar{\nu}_{\mu})\cdot \frac{B(\Lambda_c^+ \rightarrow p K^- \pi^+)}{5\%} < 2.5 \times 10^{-4}$, $B(B^- \rightarrow \Lambda_c^+ \bar{p} \ell^- \bar{\nu}_{\ell})\cdot \frac{B(\Lambda_c^+ \rightarrow p K^- \pi^+)}{5\%} < 1.0 \times 10^{-4}$. These results are in slight tension with predictions based on the measurement of $B^- \rightarrow \bar{p} p \ell^- \bar{\nu}_{\ell}$ and $B^- \rightarrow \Lambda_c^+ \bar{p} \pi^-$.

==> babarsym.tex <==
%%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised   05/22/01 P. Dauncey     Added \hepex, etc. and clean up a bit
%%%%%   Revised   12/07/00 D. Hitlin      Added features of D. Kirkby's HEP.sty
%%%%%   Revised   07/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised   07/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised   07/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised   07/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised   07/01/00 D. MacFarlane
%%%%%   Revised   06/21/00 D. Hitlin
%%%%%   Original  06/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}
\def\mupm        {\ensuremath{\mu^{\pm}}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace}
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace}
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\BBbar   {\ensuremath{B\Bbar}\xspace} 
\def\BBb     {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\BzBzbar {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}

% added by GHM on March 25, 2003 -- from Andrei Gritsan
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% TAU BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\cal B}\xspace}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace}

\def\BtoDK      {\ensuremath{B \to DK}\xspace}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace}

\def\Btoetah    {\ensuremath{B \to \eta h}\xspace}
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace}

\def\btosgam    {\ensuremath{b \to s \g}\xspace}
\def\btodgam    {\ensuremath{b \to d \g}\xspace}
\def\btosll     {\ensuremath{b \to s \ellell}\xspace}
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace}
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace}
\def\btosglue   {\ensuremath{b \to s g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\rm t}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}} 
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}} 
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}} 
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}} 
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}} 
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}} 
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}} 
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}} 
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}} 
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}} 
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
%\def\mum  {\ensuremath{{\rm \,\mum}}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
%\def\muma {\ensuremath{\rm \,\mum}^2\xspace}
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees


%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}


\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

%\renewcommand{\bar}[1]{\overline{#1}}  

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}\xspace}     
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


% Data processing
\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace}
\def\hertz	{\ensuremath{{\rm \,Hz}}\xspace}
\def\khertz      {\ensuremath{{\rm \,kHz}}\xspace}
%




% QCD parameters

\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}


% CKM, CP violation

\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
%\def\CPT               {\ensuremath{C\!P\!T}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!
% added by GHM on March 25, 2003
\def\C       {\ensuremath{C}\xspace}
\def\P       {\ensuremath{P}\xspace}
\def\T       {\ensuremath{T}\xspace}



\def\epstag  {\ensuremath{\varepsilon_{\rm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\cal D}\xspace}
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}






% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
%\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
%\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
%\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
%\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
%\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Meth.\xspace}
\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ A\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ B\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ C\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ D\xspace}
\newcommand{\nimBaseE}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ E\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instrum.\ and Methods~{\bf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimaa}       [1]  {\nimBaseE~{\bf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instrum.\ Methods~{\bf A{\bf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseA~{\bf #1}}
\newcommand{\nimb}      [1]  {\nimBaseB~{\bf #1}}
\newcommand{\nimc}      [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimd}      [1]  {\nimBaseD~{\bf #1}}
\newcommand{\nime}      [1]  {\nimBaseE~{\bf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\bf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\Root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% My Definitions %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\gluon  {\ensuremath{g}\xspace}

\def\pion   {\ensuremath{\pi}\xspace}

\def\LC    {\ensuremath{\Lambda_{c}}\xspace}
\def\LCs   {\ensuremath{\Lambda_{c}}\mbox{-Baryonen}\xspace}
\def\LCp   {\ensuremath{\Lambda_{c}^{+}}\xspace}
\def\LCbar {\ensuremath{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}^{-}_{c}\xspace}}
\def\LCm   {\ensuremath{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}^{-}_{c}\xspace}}            
\def\LCpm  {\ensuremath{\Lambda_{c}^{\pm}}\xspace}
\def\LCmp  {\ensuremath{\Lambda_{c}^{\mp}}\xspace}
\def\LCpi  {\ensuremath{\Lambda_{c}\pion}\xspace}

\def\pkpi {\ensuremath{\proton\Km\pip}\xspace}
\def\mpkpi {\ensuremath{m\left(\proton\Km\pip\right)}\xspace}
\def\antipkpi {\ensuremath{\antiproton\Kp\pim}\xspace}

\def\chiq {\ensuremath{\chi^{2}}\xspace}

\def\BBbar{\ensuremath{\B {\kern -0.16em \Bbar}}\xspace}

\def\SigmaC {\ensuremath{\Sigma_{c}}}
\def\Sigmac {\ensuremath{\Sigma_{c}}}
\def\SigmaCz {\ensuremath{\Sigma_{c}^{0}}}
\def\Sigmacz {\ensuremath{\Sigma_{c}^{0}}}
\def\SigmaCplplz {\ensuremath{\Sigma_{c}^{++/0}}}
\def\Sigmacplplz {\ensuremath{\Sigma_{c}^{++/0}}}
\def\SigmaCplpl {\ensuremath{\SigmaC^{++}}}
\def\Sigmacplpl {\ensuremath{\SigmaC^{++}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% My Baryon DECAYS  %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\def\lcpkpipi {\ensuremath{\LCp \antiproton \pip \pim}\xspace}

\def\LCtopkpipm {\ensuremath{\LCpm \to \proton^{\pm} \Kmp \pipm}\xspace}
\def\LCtopkpip {\ensuremath{\LCp \to \proton \Km \pip}\xspace}
\def\LCtopkpim {\ensuremath{\LCm \to \antiproton \Kp \pim}\xspace}

\def\Btolcppipi {\ensuremath{\Bzb \to \LCp \antiproton \pip \pim}\xspace}
\def\antiBtolcppipi {\ensuremath{\Bz \to \LCp \antiproton \pip \pim}\xspace}
\def\Btoantilcppipi {\ensuremath{\Bz \to \LCm \proton \pip \pim}\xspace}
\def\Btolcppipiplmi {\ensuremath{\Bzb \to \LCpm \proton^{\mp} \pipm \pimp}\xspace}
\def\mLCpi {\ensuremath{m\left(\LC\pi\right)}\xspace}
\def\mLCpip {\ensuremath{m\left(\LCp\pip\right)}\xspace}
\def\mLCpim {\ensuremath{m\left(\LCp\pim\right)}\xspace}

\def\umbruch {\penalty 0}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% My Baryon Lambda DECAYS  %%%%%%%%%%%%%%%%%%
\def\Lambdaz    {\ensuremath{\Lambda^{0}}\xspace}

\def\Bmtolppipi {\ensuremath{\Bm \to \Lambda \antiproton \pip \pim}\xspace}
\def\Bptolppipi {\ensuremath{\Bp \to \Lbar \proton \pim \pip}\xspace}

\def\Bztolppiz {\ensuremath{\Bzb \to \Lambda \antiproton \pip}\xspace}
\def\Bmtolppi {\ensuremath{\Bm \to \Lambda \antiproton \piz}\xspace}

\def\BmtollK {\ensuremath{\Bm \to \Lambda \Lbar \Kp}\xspace}
\def\Bmtollp {\ensuremath{\Bm \to \Lambda \Lbar \pip}\xspace}


\def\Bmtolp {\ensuremath{\Bm \to \Lambda \antiproton}\xspace}
\def\Bztoll {\ensuremath{\Bzb \to \Lambda \Lbar}\xspace}


\def\Bztolppipipi {\ensuremath{\Bzb \to \Lambda \antiproton \pip \pim \pip}\xspace}

\def\Bmtolcppiz {\ensuremath{\Bm \to \LCp \antiproton \pim}\xspace}
\def\LCtolp  {\ensuremath{\LCp \to \Lambda \pip}\xspace}

%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: "babarsym"
%%% End: 


==> chapters/BDT_training.tex <==
For the training the Monte Carlo samples are scaled to \texttt{OnPeak} luminosity, and signal Monte Carlo is scaled to the expectation derived from $\Bm \ra \LCp \antiproton \pim$. The scaling factors are given in Table \ref{tab:scaling_MLP}.
\begin{table}
  \begin{center}
  \caption{Scaling factors for input Monte Carlo sets for the MLP training. Given are the Monte Carlo mode, the corresponding SP number and the scaling factor.}
  \begin{tabular}{ccc}\toprule
    Monte Carlo mode 	& SP number 	& scaling factor 	\\\midrule
    $uds$ 		& 998 		& $0.405$		\\
    $c\bar{c}$		& 1005		& $0.489$		\\
    generic $\BpBm$	& 1235		& $0.333$		\\
    generic $\BzBzb$	& 1237		& $0.329$		\\
    $\Bp \ra \eta_b \ep \nue$ & 11455	& $0.015$		\\
    $\Bm \ra \eta_b \en \nueb$ & 11456	& $0.015$		\\
    $\Bp \ra \eta_b \mup \num$ & 11457	& $0.014$		\\
    $\Bm \ra \eta_b \mun \numb$ & 11458	& $0.014$		\\\bottomrule
  \end{tabular}
  \label{tab:scaling_MLP}
  \end{center}
\end{table}
For the electron channel the obtained ROC curve, i.e. background rejection efficiency vs. signal efficiency can be seen in Fig. \ref{fig:training_electron}, as well as the discriminator variable, given by the neural net.
\begin{figure}[h]
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/training/electron/ROC_curve}
    \label{subfig:ROC_electron}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/training/electron/Classifier_dist}
    \label{subfig:Classifier}
  }
  \caption{ROC curve \subref{subfig:ROC_electron} and classifier distribution \subref{subfig:Classifier} for the MLP training for the electron channel.}
  \label{fig:training_electron}
\end{figure}

==> chapters/CleanUp.tex <==
In order to reduce the number of wrongly or poorly reconstructed \B candidates several clean-up requirements are applied to the reconstructed \B candidates.


==> chapters/Gutachter.tex <==
\vspace*{\fill}
{\bf Gutachter:}
\begin{enumerate}
  \item Priv.-Doz. Dr. Roland Waldi \\ Institut f\"ur Physik, Universit\"at Rostock
  \item Prof. Dr. Wolfgang Gradl \\ Institut f\"ur Kernphysik, Johannes-Gutenberg-Universit\"at Mainz
\end{enumerate}
\vspace{2mm}
{\bf Datum der Einreichung:} 21. August 2014\\
{\bf Datum der Verteidigung:} 19. Dezember 2014
% \vskip 1.5em
%\begin{tabular}{ll}
%Tag der Anmeldung: & ??? \\
%Tag der Abgabe:    & ??? \\
%\end{tabular}

==> chapters/MLP_explained.tex <==
For the later discrimination of background against signal we use a neural net, more specifically a multi layer perceptron (MLP).The MLP is the most commonly used implementation of a neural net in physics. Its primary goal is to optimally separate classes of events, in this case background and signal events. The central part of the MLP is the perceptron, an algorithmic analogy of the neuron. 
The input of a perceptron is an $n$-dimensional vector $\vec{x}$, where the components $x_i$ represent different input variables, to which the perceptron has to react to.
The input vector $\vec{x}$ is weighted and shifted with the weight vector $\vec{w}$ and the response of the perceptron is determined by its activation function $y$.

Commonly used activation functions are:
\begin{itemize}
  \item the binary threshold function - returns $0$ if $\vec{w}\cdot\vec{x} \leq 0$ and $1$ if $\vec{w}\cdot\vec{x}>0$
  \item a sigmoid, given by $\displaystyle y = \frac{1}{1+e^{\vec{w}\cdot\vec{x}}}$, with output values in the range of $0$ to $+1$
  \item the hyperbolic tangent $y =\tanh{\vec{w}\cdot\vec{x}}$, with output values in the range of $-1$ to $+1$
  \item the radial function$y = e^{-\vec{w}\cdot\vec{x}}$, with output values in the range of $0$ to $+1$
\end{itemize}
While the binary threshold function represents a sharp distinction between signal and background the other functions allow for events that are only, e.g. $10\%$ signal-like.

Using only one perceptron results in defining a plane $\vec{w}\cdot\vec{x}$ in an $n$-dimensional space with signal events on one side of the plane and background events on the other side. In turn the use of a single perceptron cannot perform better than a cut-based selection.

A multi layer perceptron consists of $n$ layers of perceptrons. Here, each perceptron of the layer $n+1$ is connected to each perceptron of the layer $n$. The general implementation for the classification signal/background is an input layer with $n$ perceptrons, each with one input variable. After the input layer $m$ hidden layers with different numbers of perceptrons follow. The last layer is represented by a single perceptron, which gets the output values of each perceptron of the last hidden layer. The output of this last perceptron is then used to discriminate between signal and background.

==> chapters/MLP_select.tex <==
The TMVA package provides in addition to the MLP framework a tool to determine the best selection cut, based on the expected number of background events as well as the expected number of signal events. In order to determine the first one, the number of background events we rely on Monte Carlo events. Therefore we define a signal region in the \mes-\DeltaE plane. As seen in Figure \ref{fig:DeltaEmESplaneSignalMC} the signal has a localized peak at the nominal \B values with large tails. For a good signal separation we define our signal region as $\pm 3 \sigma$ of the localized peak. To determine the values for $\sigma$ we fit \DeltaE and \mes, with an {\it ad-hoc} signal window in the other variable. For the \DeltaE fit we require $\mes > 5.27\gevcc$.

==> chapters/MLP_training.tex <==
The selected MLP layout is a three layer design, with 9 input neurons, a hidden layer with 15 neurons and a single output neuron. For the training the Monte Carlo samples are scaled to \texttt{OnPeak} luminosity, and signal Monte Carlo is scaled to the expectation derived from $\Bm \ra \LCp \antiproton \pim$. The scaling factors are given in Table \ref{tab:scaling_MLP}.
\begin{table}
  \begin{center}
  \caption{Scaling factors for input Monte Carlo sets for the MLP training. Given are the Monte Carlo mode, the corresponding SP number and the scaling factor.}
  \begin{tabular}{ccc}\toprule
    Monte Carlo mode 	& SP number 	& scaling factor 	\\\midrule
    $uds$ 		& 998 		& $0.405$		\\
    $c\bar{c}$		& 1005		& $0.489$		\\
    generic $\BpBm$	& 1235		& $0.333$		\\
    generic $\BzBzb$	& 1237		& $0.329$		\\
    $\Bp \ra \eta_b \ep \nue$ & 11455	& $0.015$		\\
    $\Bm \ra \eta_b \en \nueb$ & 11456	& $0.015$		\\
    $\Bp \ra \eta_b \mup \num$ & 11457	& $0.014$		\\
    $\Bm \ra \eta_b \mun \numb$ & 11458	& $0.014$		\\\bottomrule
  \end{tabular}
  \label{tab:scaling_MLP}
  \end{center}
\end{table}
For the electron channel the obtained ROC curve, i.e. background rejection efficiency vs. signal efficiency can be seen in Fig. \ref{fig:training_electron}, as well as the discriminator variable, given by the neural net.
\begin{figure}[h]
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/training/electron/ROC_curve}
    \label{subfig:ROC_electron}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/training/electron/Classifier_dist}
    \label{subfig:Classifier}
  }
  \caption{ROC curve \subref{subfig:ROC_electron} and classifier distribution \subref{subfig:Classifier} for the MLP training for the electron channel.}
  \label{fig:training_electron}
\end{figure}

To study the influence of the off-set between data and Monte Carlo seen in the previous section we trained the neural net on \texttt{OnPeak} data, this study can be found in appendix \ref{sect:app:DataDrivenMLP}.

The ROC curve, as well as the discriminator variable for the \B decay via the muon can be seen in Fig. \ref{fig:training_electron}.
\begin{figure}[h]
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/training/muon/ROC_curve}
    \label{subfig:ROC_muon}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/training/muon/Classifier_dist}
    \label{subfig:Classifier_muon}
  }
  \caption{ROC curve \subref{subfig:ROC_muon} and classifier distribution \subref{subfig:Classifier_muon} for the MLP training for the muon channel.}
  \label{fig:training_muon}
\end{figure}

==> chapters/TMVA_input.tex <==
% For the final thesis this chapter should probably contain only the selected method, with an in detail explanation
Based on the analyses of $\B \ra \pi \ell \nu$, $\B \ra \rho \ell \nu$ \cite{BAD1520,PhysRevD:83:032007} and $\Bm \ra D_s^+ \Km \ellm \nulb$ \cite{BAD2183} we decide to use the following variables for the discrimination of background against signal. In addition we use the fit probability for the $Y$ vertex. For the particle ID used in this calculation we use the same algorithm as described in section \ref{sect:nu_reco}.
\begin{itemize}
  \item $L2$, defined as $L2=\sum_i|\vec{p}_i^*|\cos^2\theta_i^*$, where the sum incorporates all tracks in the event, except the $Y$ candidate. Here, $\vec{p}_i^*$ and $\theta_i^*$ are measured in the CMS with respect to the $Y$ thrust axis;
  \item $R2$, the second normalixzed Fox-Wolfram moment;
  \item $|\cos\Delta\theta_{\rm thrust}|$, the cosine of the angle between the $Y$ thrust axis and the thrust axis of the rest of the event;
  \item $P_Y(\chi^2)$, the probability that the $Y$ daughters come from a common vertex;
  \item $cos\theta_{BY}$ as defined in Eq. \ref{eq:cosBY};
  \item $\theta_{\rm miss}$, the missing polar angle;
  \item $p_{\rm miss}$, the momentum of the neutrino;
\end{itemize}

A comparison between background Monte Carlo, \texttt{OnPeak} data and signal Monte Carlo (the \texttt{JETSET42} model) can be found in Fig. \ref{fig:comp_TMVA_input_electron} for the electron channel and in Fig. \ref{fig:comp_TMVA_input_muon} for the muon channel. The obvious feature of all given figures is a discrepancy between the \texttt{OnPeak} data and the Monte Carlo distributions. This might be due to a wrongly calculated scaling of the Monte Carlo modes, or more likely due to the insufficient modeling of baryonic \B decays in the generic \B Monte Carlo.

In order to avoid a bias in the latter signal yield extraction we study the correlation with \DeltaE. The corresponding plots for the electron channel are shown in Fig. \ref{fig:corr_TMVA_input_electron}. Since none of the variables shows a correlation with \DeltaE for the signal Monte Carlo mode all variables can be used for background reduction.
\begin{figure}[h]
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/CorrelationPlots/electron/L2_DeltaE_corr}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/CorrelationPlots/electron/R2_DeltaE_corr}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/CorrelationPlots/electron/cosDthr_DeltaE_corr}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/CorrelationPlots/electron/cosBY_DeltaE_corr}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/CorrelationPlots/electron/YcandFitprob_DeltaE_corr}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/CorrelationPlots/electron/thetamiss_DeltaE_corr}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/CorrelationPlots/electron/pmiss_DeltaE_corr}
  }
  \caption{Comparison of the different background sources with signal Monte Carlo for $\Bm \ra \LCp \antiproton \en \nueb$ for the input variables for the TMVA methods.}
  \label{fig:corr_TMVA_input_electron}
\end{figure}

==> chapters/TMVA_training.tex <==
In order to decide on a MVA method we tested the two most prominent methods for the electron channel. A multi-layer perceptron (MLP), an implementation of a neural net, and boosted decision trees (BDT) with different boosting methods. The detailed implementations are as follows:
\begin{itemize}
  \item Multi-layer perceptron
    \begin{enumerate}
      \item Sigmoid neurons; 1 hidden layer with 15 neurons
    \end{enumerate}
  \item Boosted decision tree (400 trees)
    \begin{enumerate}
      \item Bagged (BDTBag)
      \item Adaptive Boost (BDTAdaBoost)
      \item Gradient Boost (BDTGradBoost)
    \end{enumerate}
\end{itemize}
The resulting signal efficiency vs. background reduction curve (ROC curve) is shown in Fig. \ref{fig:electron:comp:TMVA:methods}. As it can be seen from the graph all methods, except the bagged decision tree, have a similar performance. We decide to use the adaptive boost BDT for the benefit of a short training duration.
\begin{center}
  \begin{figure}[h]
    \centering\includegraphics[width=.6\textwidth]{figures/TMVA/compare/electron/ROC_methods}
    \caption{Comparison of different MVA methods. Shown is the background rejection vs. the signal efficiency of the different methods for the decay $\Bm \ra \LCp \antiproton \en \nueb$.}
    \label{fig:electron:comp:TMVA:methods}
  \end{figure}
\end{center}

==> chapters/dank.tex <==
\thispagestyle{empty}
\subsection*{Danksagung}

Ich bedanke mich bei der Arbeitsgruppe Elementarteilchenphysik Rostock, die es mir ermöglicht hat diese Arbeit zu schreiben.
Insbesondere möchte ich mich bei Privatdozent Roland Waldi f\"ur die gute Betreuung bedanken. 
Weiterhin bedanke ich mich bei meinen Arbeitskollegen für die Unterstützung und Gesell\-schaft. Besonderer Dank gilt hierbei Christian Vo{\ss}, der stets bereit war mit mir auf Fehler- oder Erklärungssuche zu gehen.\\
Außerdem möchte ich mich bei der \babar Kollaboration bedanken für die kompetente Hilfe in den Hypernewsforen, sowie den guten Computing-Support.\\
Des weiteren bedanke ich mich bei meiner Freundin und meiner Familie, ohne die diese Arbeit nicht möglich gewesen wäre, sie haben mich stets unterstützt.\\
Auch meinen Freunden schulde ich Dank, für das gemeinsame mensen, die Diskussionen und ihre Freundschaft. Zu guter Letzt m\"ochte ich mich bei Alex und Thomas f\"ur die abschlie{\ss}ende Kontrolle dieser Arbeit bedanken.


==> chapters/erklaerung.tex <==
\thispagestyle{empty}
{\bf Doktoranden-Erkl\"arung gem\"a{\ss} \S 4 Absatz 1 Buchstaben g und h der Promotionsordnung der Mathematisch-Naturwissenschaftlichen Fakult\"at der Universit\"at Rostock}

\bigskip

\begin{tabular}{ll}
        {\it Name}      & Leddig, Torsten \\
        {\it Anschrift} & Kleine M\"onchenstr. 2, 18055 Rostock
\end{tabular}

Ich habe eine Dissertation zum Thema

\begin{center}
        {\bf {\it Search for the decay $\Bm \ra \LCp \antiproton \ellm \nulb$ with the \babar Detector}}
\end{center}

an der Mathematisch-Naturwissenschaftlichen Fakult\"at der Universit\"at Rostock angefertigt. Dabei wurde ich von Herrn {\bf Dr. Roland Waldi} betreut.

Ich gebe folgende Erkl\"arung ab:
\begin{enumerate}
        \item Die Gelegenheit zum vorliegenden Promotionsvorhaben ist mir nicht kommerziell vermittelt worden. Insbesondere habe ich keine Organisation eingeschaltet, die gegen Entgelt Betreuerinnen/Betreuer f\"ur die Anfertigung von Dissertationen sucht oder die mir obliegenden Pflichten hinsichtlich der Pr\"ufungsleistungen f\"ur mich ganz oder teilweise erledigt.
        \item Ich versichere hiermit an Eides statt, dass ich die vorliegende Arbeit selbst\"andig angefertigt und ohne fremde Hilfe verfasst habe. Dazu habe ich keine au{\ss}er den von mir angegebenen Hilfsmitteln und Quellen verwendet und die den benutzten Werken inhaltlich und w\"ortlich entnommenen Stellen habe ich als solche kenntlich gemacht.
%        \item Die Arbeit wurde bisher weder im Inland noch im Ausland in gleicher oder \"ahnlicher Form
%einer anderen Pr\"ufungsbeh\"orde vorgelegt.
\end{enumerate}

\vskip 1cm

Rostock, den 22. August 2014

% \vspace*{35\baselineskip}
% \hbox to \textwidth{\hrulefill}
% \par
% Ich erkläre hiermit, dass ich die vorliegende Arbeit selbständig verfasst und
% keine anderen als die angegebenen Quellen und Hilfsmittel verwendet habe.

% Rostock, den ...

\clearpage







%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: "diplarb"
%%% End: 


==> chapters/fit_procedure.tex <==
For the signal extraction in \mes we have to find a good description of the background and signal description. Therefore we fit background with an Argus fuction, defined as
\[\]

==> chapters/fit_to_data.tex <==
We determine the signal yield in data by using the fit functions described in the previous section. For the fit itself we fix all parameters, except the signal and background yields to the values obtained in the fits to signal and background Monte Carlo. The fitted \DeltaE distributions for \texttt{OnPeak} data can be see in Fig. \ref{fig:DeltaE_fitToData}.
\begin{figure}[h]
  \subfigure[]{  \includegraphics[width=.48\textwidth]{figures/TMVA/cut/eChannel_Fit_OnPeak_DeltaE}
    \label{fig:DeltaE_fitToData_electron}
  }
  \subfigure[]{  \includegraphics[width=.48\textwidth]{figures/TMVA/cut/muChannel_Fit_OnPeak_DeltaE}
    \label{fig:DeltaE_fitToData_muon}
  }
  \caption{Fitted \DeltaE distributions in \texttt{OnPeak} data.\subref{fig:DeltaE_fitToData_electron} shows the fit for the electron channel, and \subref{fig:DeltaE_fitToData_muon} shows the fit for the muon channel.}
  \label{fig:DeltaE_fitToData}
\end{figure}

From the fits we obtain signal yields of
\begin{equation}
  \begin{split}
    N_{\rm sig}(\Bm \ra \LCp \antiproton \en \nueb)  &= 0 \pm 21 \\
    N_{\rm sig}(\Bm \ra \LCp \antiproton \mun \numb) &= 20 \pm 60.
  \end{split}
  \label{eq:Nsig_data}
\end{equation}
The log-likelihoods for the fits are $7.81$ and $7.42$ respectively.
As can be seen from the fits shown in Fig. \ref{fig:DeltaE_fitToData} no isolated signal peak is visible. The sensitivity of the fit for signal comes primarily from the peak position of the total distribution. This method relies strongly on the Monte Carlo description of signal and background, which we assume to be correct.

==> chapters/fit_variable.tex <==
For signal extraction we have to decide between two different variables, \mes and \DeltaE. The common variables $M_{\rm miss}^2$ and $M_{\rm miss}^2/2E_{\rm miss}$ cannot be used due to the large invariant mass of the $Y$ system, constraining the energy release by the neutrino to small values. In consequence $M_{\rm miss}^2/2E_{\rm miss}$ tends to diverge, while $M_{\rm miss}^2$ peaks at $0\gev^2/c^4$ for background as well, and thus would be suitable for tagged analyses only.
The two-dimensional \DeltaE:\mes distributions for WI signal Monte Carlo and background Monte Carlo for the electron channel are shown in Fig. \ref{fig:2D_SigAndBkg_eChannel}.
\begin{figure}[h]
        \subfigure[]{
                \includegraphics[width=.48\textwidth]{figures/target/DeltaE_mES_sig_eChannel}
                \label{subfig:sig_2D}
        }
        \subfigure[]{
                \includegraphics[width=.48\textwidth]{figures/target/DeltaE_mES_bkg_eChannel}
                \label{subfig:bkg_2D}
        }
        \caption{\DeltaE:\mes plane for \subref{subfig:sig_2D} WI signal Monte Carlo, and \subref{subfig:bkg_2D} background Monte Carlo. The signal Monte Carlo is scaled to an expected branching fraction of $1\cdot 10^{-4}$. The background Monte Carlo is a mixture of $q\bar{q}$ and $\BBb$ Monte Carlo, scaled to data luminosity individually.}
        \label{fig:2D_SigAndBkg_eChannel}
\end{figure}
The small number of signal events in the peak for WI signal Monte Carlo shows that we will be able to determine only an upper limit for the signal decay, if its branching fraction is at the order of $10^{-4}$ as we expect.

For the one-dimensional fit we decide to cut in \DeltaE and fit in \mes, since background as well as signal  show a broad, but peaked distribution in \DeltaE, making it difficult to distinguish background from signal in this variable. We determine the \DeltaE cut by constraining \mes to values larger than $5.25\gevcc$ and fitting \DeltaE with a Cruijff function, defined as
\begin{align}
  \label{eq:cruijff}
  \begin{split}C(x;m_0, \sigma_L, \sigma_R, \alpha_L, \alpha_R) =
\begin{cases}
    \exp\left(-\frac{(x-m_0)^2}{2(\sigma_{L}^2+\alpha_{L}(x-m_0)^2)}\right)
    & \mbox{if } x<m_0 \\
    \exp\left(-\frac{(x-m_0)^2}{2(\sigma_{R}^2+\alpha_{R}(x-m_0)^2)}\right)
    & \mbox{if } x>m_0. \\
\end{cases}\end{split}
\end{align}
\begin{figure}[h]
  \begin{center}
    \subfigure[]{
      \includegraphics[width=.48\textwidth]{figures/TMVA/cut/eChannel_DeltaE_sig_bestCut_fit}
      \label{fig:clf_opt_eChannel_fit_sig}
    }
    \subfigure[]{
      \includegraphics[width=.48\textwidth]{figures/TMVA/cut/muChannel_DeltaE_sig_bestCut_fit}
      \label{fig:clf_opt_muChannel_fit_sig}
    }
  \end{center}
  \caption{Fitted signal \DeltaE distribution for the electron \subref{fig:clf_opt_eChannel_fit_sig} and the muon \subref{fig:clf_opt_muChannel_fit_sig} channel. In both cases signal is fitted with a Cruijff function.}
  \label{fig:sig_cruijff_fit}
\end{figure}
\begin{tabular}{lr}
  \begin{minipage}{.46\textwidth}
    \begin{table}[H]
      \caption{Fit parameter for the \DeltaE fit in WI signal Monte Carlo for the electron channel.}%FCN = 14.2157542848
      \begin{center}
      \begin{tabular}{lc}
        \toprule
        parameter & value \\\midrule
        $m_{0} $ & $ 0.012 \pm 0.008$\\
        $\sigma_L $ & $ 0.389 \pm 0.007$\\
        $\sigma_R $ & $ 0.542 \pm 0.009$\\
        $\alpha_L$ & $0.213 \pm 0.005$\\
        $\alpha_R$ & $0.170 \pm 0.007$\\
        $N_{\rm sig}$ & $67830 \pm 270$\\
        \bottomrule
      \end{tabular}
      \end{center}
      \label{tab:fitDeltaE_sig_eChannel}
    \end{table}
  \end{minipage} &
  \begin{minipage}{.46\textwidth}
    \begin{table}[H]
      \caption{Fit parameter for the \DeltaE fit in WI signal Monte Carlo for the muon channel.}
      \begin{center}
        \begin{tabular}{lc}\toprule
          parameter & value \\\midrule
          $m_{0} $ & $ 0.053 \pm 0.009$\\
          $\sigma_L $ & $ 0.414 \pm 0.008$\\
          $\sigma_R $ & $ 0.531 \pm 0.010$\\
          $\alpha_L$ & $0.204 \pm 0.006$\\
          $\alpha_R$ & $0.174 \pm 0.008$\\
          $N_{\rm sig}$ & $61340 \pm 250$\\
          \bottomrule
        \end{tabular}
      \end{center}
      \label{tab:fitDeltaE_sig_muChannel}
    \end{table}
  \end{minipage}
\end{tabular}
For the latter \mes fit we use an asymmetric $3\sigma$ cut in \DeltaE, based on the fit results given in Table \ref{tab:fitDeltaE_sig_muChannel}. For the electron channel this translates into
\begin{equation}
        -1.17 < \DeltaE < 1.63 \gev,
\end{equation}
and for the muon channel
\begin{equation}
        -1.24 < \DeltaE < 1.59 \gev.
\end{equation}


==> chapters/motivation.tex <==
\B mesons are the lightest mesons with a substantial contribution to the total branching fraction from decays to baryons. For \BpBm/\BzBzb mesons the ARGUS collaboration measured an inclusive branching fraction of $(6.8 \pm 0.5_{\rm stat} \pm 0.3_{\rm syst})\%$ for the decay into baryons \cite{Albrecht:1992he}. In the last decade the \B-factories measured a large variety of such decays, shedding light on the underlying processes. The experiments discovered some puzzling features of baryonic \B decays, like the threshold enhancement, or the preference for higher multiplicities.


==> chapters/neutrino_theta.tex <==
A source for fake signal events, are events where one or more particles are lost down the beampipe, missing all active detector regions. A feature of this events would be a missing momentum vector pointing towards the inactive detector regions around the beam pipe. Thus, requiring the missing polar angle to be within the interval $[0.41,\, 2.37]$, representing the active and well calibrated part of the detector. A comparison of $\theta_{\rm miss}$ for signal and background can be seen in Fig. \ref{fig:ThetaMiss}. The comparison shows that signal and background have a rather similar behavior, and in turn a cut on $\theta_{\rm miss}$ would reduce the background as well as the signal. For this reason we decide not to apply a selection in $\theta_{\rm miss}$.
% To avoid these candidates we require the missing polar angle $\theta_{\rm miss}$ to be within the active detector volume
% \begin{equation}
%   0.41 < \theta_{\rm miss} < 2.37 \,{\rm rad}.
% \end{equation}
% A comparison of the polar angle distribution for signal and background can be found in Fig. \ref{fig:ThetaMiss}.
\begin{figure}[h]
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/compareVariables/electron/ThetaMiss}
    \label{fig:electron:ThetaMiss}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/compareVariables/muon/ThetaMiss}
    \label{fig:muon:ThetaMiss}
  }
  \caption{Missing polar angle for the $\LCp \antiproton \en \nueb$ \subref{fig:electron:ThetaMiss} and $\LCp \antiproton \mun \numb$ \subref{fig:muon:ThetaMiss} channel. Background Monte Carlo data sets are stacked, \texttt{OnPeak} data and signal Monte Carlo are super-imposed.}
  \label{fig:ThetaMiss}
\end{figure}

Another source for fake signal events are fully reconstructed events, with a misidentified lepton. Especially for the muon case mis-identified pions can fake a signal event. What is common to fully reconstructed events, is a small missing momentum, thus the requirement of a minimum missing momentum should reduce this problem. A comparison of signal and background is shown in Fig. \ref{fig:pMiss}. Both distributions show a peak at lower values for background than for signal. A conservative cut, derived from these distributions would be
\begin{equation}
  |\vec{p}|_{\rm miss} > 0.8 \gevc\, .
\end{equation}
\begin{figure}[h]
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/compareVariables/electron/pMiss}
    \label{fig:electron:pMiss}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/compareVariables/muon/pMiss}
    \label{fig:muon:pMiss}
  }
  \caption{Missing momentum for the $\LCp \antiproton \en \nueb$ \subref{fig:electron:pMiss} and $\LCp \antiproton \mun \numb$ \subref{fig:muon:pMiss} channel. Background Monte Carlo data sets are stacked, \texttt{OnPeak} data and signal Monte Carlo are super-imposed.}
  \label{fig:pMiss}
\end{figure}
A cut on the missing momentum shows two problems, first the momentum distribution in Monte Carlo depends on the chosen model for simulation. Since there is no theoretical expectation on this decay the model is highly phenomenological, trying to describe one of the most common feature in baryonic \B decays. Second, the missing momentum is strongly correlated with \DeltaE, the selected variable for signal extraction. Thus, a cut in $|\vec{p}_{\rm miss}|$ might spoil the \DeltaE distribution for background.


==> chapters/peakingBkg.tex <==
Applying the previously defined cut on the Random Forest output distribution we obtain the \DeltaE distributions shown in Fig. \ref{fig:DeltaE_clfCut}. Both distributions show an agreement between data and Monte Carlo on the level of $1\sigma$, possible discrepancies could arise from the uncertainty on the scaling to data luminosity. There is no sign of an additional signal peak in this distribution. But, since generic $B\bar{B}$ Monte Carlo is known to poorly model baryonic \B decays\footnote{all baryonic modes are generated by \texttt{JETSET}, with an arbitrary branching fraction}, we study the contributing decay modes in the \B Monte Carlo.
\begin{figure}[h]
  \subfigure[]{
    \includegraphics[width=.47\textwidth]{figures/TMVA/training/DeltaE_eChannel_clfCut}
    \label{subfig:clf_Cut_e}
  }
  \subfigure[]{
    \includegraphics[width=.47\textwidth]{figures/TMVA/training/DeltaE_muChannel_clfCut}
    \label{subfig:clf_Cut_mu}
  }
  \caption{Stacked \DeltaE distributions for $q\bar{q}$ and $\BBb$ background overlayed with the distribution obtained from \texttt{OnPeak} data. For \subref{subfig:clf_Cut_e} $\Bm \ra \LCp \antiproton \en \nueb$ and \subref{subfig:clf_Cut_mu} $\Bm \ra \LCp \antiproton \mun \numb$.}
  \label{fig:DeltaE_clfCut}
\end{figure}

==> chapters/peaking_background.tex <==
l

==> chapters/rf_inputVars.tex <==
For the further background suppression we decide to use a random forest, as explained in detail in section \ref{sect:rf_explain}.
We train a random forest consisting of $500$ trees with a minimal event number of $1$ for each node and the number of variables for the split is set to $\sqrt{p}$, where $p$ is the total number of input variables. For background The size of the input datasets is chosen in such a way, that the number of background events for $q\bar{q}$ and $\BBb$ Monte Carlo in the training sample equals the number of training signal events.

\subsection{Input variables}

As input variables we decide to use the following seven variables
\begin{itemize}
  \item The ratio of the second and zeroth Fox-Wolfram moment for all charged tracks $R_2$, defined as
    \begin{equation}
      R_2 = \frac{\sum_{ij}|p_i||p_j|P_2(\cos\theta_{ij})}{\sum_{ij}|p_i||p_j|P_0(\cos\theta_{ij})},
    \end{equation}
    whith the Legendre polynomials $P_0$ and $P_2$ and the angle $\theta_{ij}$ between the momenta $p_i$ and $p_j$ \cite{Sjostrand:2006za}.
  \item The sphericity $S$ of the event, derived from the sphericity tensor
    \begin{equation}
      S^{\alpha\beta} = \frac{\sum_ip_i^{\alpha}p_i^{\beta}}{\sum_i|\vec{p}_i|^2},
    \end{equation}
    where $\alpha, \beta=1,2,3$ correspond to the $x$, $y$ and $z$ components \cite{Sjostrand:2006za}.
  \item the cosine of the angle between the thrust axis of the $Y$ candidate and the thrust axis of the rest of the event $cos\Delta\theta_{\rm thrust}$. The thrust axis is defined \cite{Sjostrand:2006za} as the vector $\vec{n}$ that maximizes the thrust $T$
    \begin{equation}
      T = \max_{|\vec{n}|=1}\frac{\sum_i|\vec{n}\cdot\vec{p}_i|}{\sum_i|\vec{p}_i|}.
    \end{equation}
  \item $p_{\ell T} = |\vec{p}(\ell)| + p_T(\nu)$
  \item the angle between the lepton momentum and the momentum of the $\LCp \antiproton$ system in the CM frame
  \item the vertex probability for the $Y$ candidate
  \item the neutrino momentum
%  \item the energy substituted mass \mes
%  \item \mes of the second \B
%  \item the energy difference \DeltaE for the second \B
\end{itemize}
The first two variables are event variables, suitable to distinguish especially jet-like $q\bar{q}$ events from signal events. A comparison of these variables for signal and background can be seen in Figure \ref{fig:comp:evtShape_eChannel}. Both distributions show a good separation of $uds$ and \ccbar from \BBbar and signal events, but no separation power between signal and \BBbar background.
\begin{figure}[h]
  \begin{center}
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/Input/R2_comp_eChannel}
    \label{subfig::comp:evtShape_eChannel:R2}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/TMVA/Input/spher_comp_eChannel}
    \label{subfig::comp:evtShape_eChannel:spher}
  }
  \end{center}
  \caption{Comparison of signal and background distributions in \subref{subfig::comp:evtShape_eChannel:R2} $R_2$ and \subref{subfig::comp:evtShape_eChannel:spher} the event sphericity $spher$ for the electron channel. The distributions have been scaled to the same integral.}
  \label{fig:comp:evtShape_eChannel}
\end{figure}

For $q\bar{q}$ events we expect that the angle between the thrust axis of the $Y$ candidate and the rest of the event is close to zero, due to the strong jet-like event topology. In contrast, for \BBbar events no such correlation is expected. This makes $\cos\Delta\theta_{\rm thrust}$ a good variable to distinguish $q\bar{q}$ background from \BBbar events. A comparison of background and signal for the electron channel can be found in Fig. \ref{fig:comp:cosDThThr_eChannel}. As expected there is a strong peak at $+1$ for $uds$ and $\ccbar$ events, while \BBbar background behaves like signal.
\begin{figure}[h]
  \begin{center}
    \includegraphics[width=.48\textwidth]{figures/TMVA/Input/cosDeltaThetaThrust_comp_eChannel}
  \end{center}
  \caption{Comparison of signal and background distributions in $\cos\Delta\theta_{\rm thrust}$ for the electron channel. The distributions have been scaled to the same integral.}
  \label{fig:comp:cosDThThr_eChannel}
\end{figure}

Comparing the two-dimensional plane $p_T(\nu):p_{\ell}$ for signal Monte Carlo and background simulation we can see a strong anticorrelation between the two quantities for signal events, leaving the lower left corner unpopulated. In contrast background events from $B\bar{B}$ and $q\bar{q}$ Monte Carlo simulations populate this corner. In consequence this plane is a good measure to distinguish signal and background. Figure \ref{fig:pT_pl_eChannel} shows this plane for signal and background Monte Carlo in the case of the electron channel. To benefit from this behavior we define the variable $p_{\ell T} = |\vec{p}(\ell)| + p_T(\nu)$, which shows a good separation of background and signal.
\begin{figure}[h]
  \subfigure[]{
  \includegraphics[width=.48\textwidth]{figures/TMVA/Input/pT_pl_eChannelqqbar}
  \label{subfig:pT_pl_eChannelqqbar}
  }
  \subfigure[]{
  \includegraphics[width=.48\textwidth]{figures/TMVA/Input/pT_pl_eChannelBBbar}
  \label{subfig:pT_pl_eChannelBBbar}
  } 
  \centering\subfigure[]{
  \includegraphics[width=.48\textwidth]{figures/TMVA/Input/pT_pl_eChannelSig}
  \label{subfig:pT_pl_eChannelSig}
  } 
  \centering\subfigure[]{
  \includegraphics[width=.48\textwidth]{figures/TMVA/Input/plT_comp_eChannel}
  \label{subfig:plT_comp_eChannel}
  } 
  \caption{Lepton momentum vs. neutrino transverse momentum for \subref{subfig:pT_pl_eChannelqqbar} $uds$ and $c\bar{c}$, \subref{subfig:pT_pl_eChannelBBbar} \BBb and \subref{subfig:pT_pl_eChannelSig} signal Monte Carlo. The resulting one-dimensional quantity $p_{\ell T}$ is shown in \subref{subfig:plT_comp_eChannel}. All plots are for the electron channel.}
  \label{fig:pT_pl_eChannel}
\end{figure}
In order to suppress background from \BBbar events we can take benefit from our specific decay model. We use the assumption that the spectator system collapses into a single meson, the $M$, which subsequently decays into $\LCp \antiproton$. In principal the $M$ should move into the opposite direction of the $\ell \nub$ system. In consequence we expect the angle between the lepton direction and the $\LCp \antiproton$ to be peaked towards $180^{\circ}$ in the CM system, assuming that the relative momentum between lepton and neutrino is small. For \BBbar background we don't expect such correlation since the most probable case is that the lepton and the $\LCp \antiproton$ system originate from different \B mesons. Comparing the cosine of this angle $cos\theta_{\LCp \antiproton, \ell}$, as shown in Fig. \ref{fig:comp:cosThLcpl_eChannel}, we see the expected behavior, with a slight enhancement at $-1$ for \BBbar events as well. This is due to the non-negligible momentum of the \B mesons in the CM frame.\newline
Another useful quantity to suppress \BBbar background is the vertex probability for the $Y$ candidate, $P_{\chi^2}(Y)$. While we expect $\LCp$, $\antiproton$ and $\ellm$ to come from the same vertex for signal events this does not hold true for background events where these three particles originate from different \B decays. In consequence we expect $P_{\chi^2}(Y)$ to peak at $0$ and to decrease exponentially for background events. For signal events we expect a constant contribution over the range of $P_{\chi^2}(Y)$. Figure \ref{fig:comp:VtxProb_eChannel} shows the $P_{\chi^2}(Y)$ distribution for the electron channel. The strong peak at $0$ for background events is clearly visible. Concentrating on the inset, showing the range from $0.1$ to $1.0$ we see that background drops to zero, while signal rises slowly.
\begin{figure}[h]
  \begin{center}
    \subfigure[]{
      \includegraphics[width=.48\textwidth]{figures/TMVA/Input/cosThLcpl_comp_eChannel}
      \label{fig:comp:cosThLcpl_eChannel}
    }
    \subfigure[]{
      \includegraphics[width=.48\textwidth]{figures/TMVA/Input/VtxProb_comp_eChannel}
      \label{fig:comp:VtxProb_eChannel}
    }
  \end{center}
  \caption{Comparison of signal and background distributions in $cos\theta_{\LCp \antiproton, \ell}$ \subref{fig:comp:cosThLcpl_eChannel} and $P_{\chi^2}(Y)$ \subref{fig:comp:VtxProb_eChannel} for the electron channel. For the latter the inset shows the range from $0.1$ to $1.0$. The distributions have been scaled to the same integral.}
  \label{fig:comp:cosThLcpl_eChannel:VtxProb_eChannel}
\end{figure}
\newline
% Further background reduction can achieved by including the neutrino momentum $|\vec{p}_{\nu}|$ (Fig. \ref{fig:comp:pNu_eChannel}) and the energy substituted mass $\mes$ (Fig. \ref{fig:comp:BmES_eChannel}) for our signal \B. While the first variable is able to distinguish events without an energetic neutrino, the second variable peaks near the \B mass for correctly reconstructed \B mesons, and in consequence is a good measure to suppress partially reconstructed candidates.
Further background reduction can be achieved by including the neutrino momentum $|\vec{p}_{\nu}|$ (Fig. \ref{fig:comp:pNu_eChannel}) to distinguish events without an energetic neutrino.
\begin{figure}[h]
  \begin{center}
%    \subfigure[]{
      \includegraphics[width=.48\textwidth]{figures/TMVA/Input/pNu_comp_eChannel}
%      \label{fig:comp:pNu_eChannel}
%    }
    % \subfigure[]{
    %   \includegraphics[width=.48\textwidth]{figures/TMVA/Input/BmES_comp_eChannel}
    %   \label{fig:comp:BmES_eChannel}
    % }
  \end{center}
  \caption{Comparison of signal and background distributions in $|\vec{p}_{\nu}|$ \subref{fig:comp:pNu_eChannel} for the electron channel. The distributions have been scaled to the same integral.}
%  \label{fig:comp:pNu_eChannel:BmES_eChannel}
  \label{fig:comp:pNu_eChannel}
\end{figure}

%The neutrino reconstruction is very sensitive to missing particles from the second \B in the final state. A good method to avoid this bias would be a tagged analysis. Unfortunately the \babar data set containing tagged events is too small to be usable for this analysis. To benefit at least partially from a reconstruction of the second \B we combine all charged and neutral particles not used in the signal \B into a second \B candidate. In order to assess the quality of this ``reconstruction'' we include \DeltaE and \mes for the second \B into the random forest. A comparison of signal and background for these quantities can be found in Fig. \ref{fig:comp:2BmES_eChannel:2BDeltaE_eChannel}.
% \begin{figure}[h]
%   \begin{center}
%     \subfigure[]{
%       \includegraphics[width=.48\textwidth]{figures/TMVA/Input/2BmES_comp_eChannel}
%       \label{fig:comp:2BmES_eChannel}
%     }
%     \subfigure[]{
%       \includegraphics[width=.48\textwidth]{figures/TMVA/Input/2BDeltaE_comp_eChannel}
%       \label{fig:comp:2BDeltaE_eChannel}
%     }
%   \end{center}
%   \caption{Comparison of signal and background distributions in $\mes$ \subref{fig:comp:2BmES_eChannel} and $\DeltaE$ \subref{fig:comp:2BDeltaE_eChannel} for the second \B in the electron channel. The distributions have been scaled to the same integral.}
%   \label{fig:comp:2BmES_eChannel:2BDeltaE_eChannel}
% \end{figure}

For the muon channel we use the same ten variables, since they show the same qualitative behavior for this mode. The comparison plots can be found in the Appendix in Fig. \ref{fig:comp:RF_inputVars_muChannel_1} and \ref{fig:comp:RF_inputVars_muChannel_2}.

\subsection{Peformance}

The random forest is trained on a data set consisting of signal events, $uds$, $\ccbar$, $\BpBm$ and $\BzBzb$ events each. After training we obtain the classifier distributions shown in Fig. \ref{fig:clf_eChannel:clf_eChannel}. For the electron, as well as the muon channel the classifier distribution shows a good separation between signal and background (including $\qqbar$ and $\BBbar$ events). The receiver operation characteristic (ROC) curve, shown in Fig. \ref{fig:ROC_eChannel:ROC_eChannel} shows a good background suppression while preserving most of the signal.
\begin{figure}[h]
  \begin{center}
    \subfigure[]{
      \includegraphics[width=.48\textwidth]{figures/TMVA/training/clf_eChannel}
      \label{fig:clf_eChannel}
    }
    \subfigure[]{
      \includegraphics[width=.48\textwidth]{figures/TMVA/training/clf_muChannel}
      \label{fig:clf_muChannel}
    }
  \end{center}
  \caption{Random Forest output distribution for the electron \subref{fig:clf_eChannel} and muon \subref{fig:clf_muChannel} channel.}
  \label{fig:clf_eChannel:clf_eChannel}
\end{figure}
\begin{figure}[h]
  \begin{center}
    \subfigure[]{
      \includegraphics[width=.48\textwidth]{figures/TMVA/training/ROC_eChannel}
      \label{fig:ROC_eChannel}
    }
    \subfigure[]{
      \includegraphics[width=.48\textwidth]{figures/TMVA/training/ROC_muChannel}
      \label{fig:ROC_muChannel}
    }
  \end{center}
  \caption{Random Forest receiver operation characteristic distribution for the electron \subref{fig:ROC_eChannel} and muon \subref{fig:ROC_muChannel} channel.}
  \label{fig:ROC_eChannel:ROC_eChannel}
\end{figure}

==> chapters/rf_inputVars_old.tex <==
For the further background suppression we decide to use a random forest, as explained in detail in section \ref{sect:rf_explain}.
We train a random forest consisting of $500$ trees with a minimal event number of $1$ for each leaf and the number of variables for the split is set to $\sqrt{p}$. For background The size of the input datasets is chosen in such a way, that the number of background events for $q\bar{q}$ and $\BBb$ Monte Carlo in the training sample equals the number of training signal events.
As input variables we decide to use the following 12 variables
\begin{itemize}
  \item the ratio of the second and zeroth Fox-Wolfram moment for all charged tracks $R_2$
  \item the sphericity of the event
  \item the cosine of the angle between the thrust axis of the $Y$ candidate and the thrust axis of the rest of the event
  \item the $x$ and $y$ component of the neutrino momentum (missing momentum)
  \item the lepton momentum
  \item the angle between the thrust axis of the event and the momentum of the
    \begin{enumerate}
      \item lepton
      \item \LCp
      \item proton
    \end{enumerate}
  \item the energy substituted mass \mes
  \item the energy difference \DeltaE
\end{itemize}
The first three variables are event variables, suitable to distinguish especially jet-like $q\bar{q}$ events from signal events.
The $x$ and $y$ component of the neutrino momentum are used to allow for a cut on the transverse momentum of the neutrino. In general we expect the transverse momentum of the neutrino candidate to be small for background events, pointing on a lost track rather than a neutrino.
The lepton momentum can be used in a similar way, comparing the two-dimensional plane $p_T(\nu):p_{\ell}$ for signal Monte Carlo and background simulation we can see a strong anticorrelation between the two quantities for signal events, leaving the lower left corner unpopulated. In contrast background events from $B\bar{B}$ and $q\bar{q}$ Monte Carlo simulations populate this corner. In consequence this plane is a good measure to distinguish signal and background. Figure \ref{fig:pT_pl_eChannel} shows this plane for signal and background Monte Carlo in the case of the electron channel.

\begin{figure}[h]
  \subfigure[]{
  \includegraphics[width=.48\textwidth]{figures/TMVA/Input/pT_pl_eChannelqqbar}
  \label{subfig:pT_pl_eChannelqqbar}
  }
  \subfigure[]{
  \includegraphics[width=.48\textwidth]{figures/TMVA/Input/pT_pl_eChannelBBbar}
  \label{subfig:pT_pl_eChannelBBbar}
  } 
  \centering\subfigure[]{
  \includegraphics[width=.48\textwidth]{figures/TMVA/Input/pT_pl_eChannelSig}
  \label{subfig:pT_pl_eChannelSig}
  } 
  \caption{Lepton momentum vs. neutrino transverse momentum for \subref{subfig:pT_pl_eChannelqqbar} $uds$ and $c\bar{c}$, \subref{subfig:pT_pl_eChannelBBbar} \BBb and \subref{subfig:pT_pl_eChannelSig} signal Monte Carlo. All plots are for the electron channel.}
  \label{fig:pT_pl_eChannel}
\end{figure}

A major source of background are $q\bar{q}$ events, where the baryon anti-baryon pair is produced in one hemisphere of the jet-like event, and the lepton in the other hemisphere. This background can be suppressed by using the thrust axis of the event to distinguish the hemisphere. If the cosine of the angle between the thrust axis and the momentum of the particle has the opposite sign for the lepton and the baryon anti-baryon pair the corresponding \B candidate is most likely a $q\bar{q}$ background event. In contrast, if the sign is the same the candidate is more likely a signal candidate. The correlation between these three quantities is a good measure to distinguish background from signal.

We decide to include \DeltaE and \mes in the random forest since background tends to peak in them as well, making a signal extraction by a fit complicated, as can be seen in Figure \ref{fig:DeltaE_clfCut}, which was obtained during an early study. In this study we excluded $\mes$ and $\DeltaE$ from the training and used the $10$ remaining variables and a pre-defined \mes cut of $5.26\gevcc$. The cut value for the random forest output was determined by maximizing $S/B$. A detailed study on generic Monte Carlo revealed that the lepton originates from $B \ra D\ell \nu$ decays, with baryons coming from the second \B. Since generic \B Monte Carlo randomly generates baryonic \B decays it is not possible to use the obtained background description, including scaling. 
%Nevertheless $\mes$ and \DeltaE still provide a good quantity to distinguish signal from background.
\begin{figure}[h]
  \subfigure[]{
    \includegraphics[width=.47\textwidth]{figures/TMVA/training/DeltaE_eChannel_clfCut}
    \label{subfig:clf_Cut_e}
  }
  \subfigure[]{
    \includegraphics[width=.47\textwidth]{figures/TMVA/training/DeltaE_muChannel_clfCut}
    \label{subfig:clf_Cut_mu}
  }
  \caption{Stacked \DeltaE distributions for $q\bar{q}$ and $\BBb$ background overlayed with the distribution obtained from \texttt{OnPeak} data, after a cut on the random forest output. For \subref{subfig:clf_Cut_e} $\Bm \ra \LCp \antiproton \en \nueb$ and \subref{subfig:clf_Cut_mu} $\Bm \ra \LCp \antiproton \mun \numb$.}
  \label{fig:DeltaE_clfCut}
\end{figure}

Using all $12$ input variables we obtain the classifier distribution shown in Fig. \ref{fig:clf_e_mu}. The classifier shows a good separation between signal and background. The receiver operation characteristic (ROC) curve shows a high efficiency for signal selection with a small mis-identification rate. The ROC curve for both distributions can be found in Fig. \ref{fig:ROC}.
\begin{figure}[h]
  \subfigure[]{
    \includegraphics[width=.47\textwidth]{figures/TMVA/training/clf_eChannel}
    \label{subfig:clf_e}
  }
  \subfigure[]{
    \includegraphics[width=.47\textwidth]{figures/TMVA/training/clf_muChannel}
    \label{subfig:clf_mu}
  }
  \caption{The random forest classifier distributions for \subref{subfig:clf_e} the electron channel, and \subref{subfig:clf_mu} the muon channel. The background distribution is shown in blue, and the signal distribution in green.}
  \label{fig:clf_e_mu}
\end{figure}
\begin{figure}[h]
  \subfigure[]{
    \includegraphics[width=.47\textwidth]{figures/TMVA/training/ROC_eChannel}
    \label{subfig:ROC_e}
  }
  \subfigure[]{
    \includegraphics[width=.47\textwidth]{figures/TMVA/training/ROC_muChannel}
    \label{subfig:ROC_mu}
  }
  \caption{The random forest classifier distributions for \subref{subfig:ROC_e} the electron channel, and \subref{subfig:ROC_mu} the muon channel. The background distribution is shown in blue, and the signal distribution in green.}
  \label{fig:ROC}
\end{figure}

%To determine the optimal cut value we integrate the classifier distributions and calculate $S/B$ for different cut values. The resulting distributions can be seen in Fig. \ref{fig:clf_opt}.
%\begin{figure}[h]
%  \subfigure[]{
%    \includegraphics[width=.47\textwidth]{figures/TMVA/training/clf_opt_eChannel}
%    \label{subfig:clf_opt_e}
%  }
%  \subfigure[]{
%    \includegraphics[width=.47\textwidth]{figures/TMVA/training/clf_opt_muChannel}
%    \label{subfig:clf_opt_mu}
%  }
%  \caption{Signal over background ratio for the electron \subref{subfig:clf_opt_e} and the muon \subref{subfig:clf_opt_mu} channel. To avoid infinities in the calculation we use $(S+1)/(B+1)$.}
%  \label{fig:clf_opt}
%\end{figure}
%For both decay channels, the electron as well as the muon mode, we find an optimal value of $0.79$ for the background suppression.


==> chapters/signal_window.tex <==
In order to reduce background further we can apply cuts in \mes and \DeltaE. As can be seen from Fig. \ref{fig:DeltaEmESplaneSignalMC} both quantities have a localized peak at the nominal values, with large radiative tails. For the muon channel the peak seems to be a bit more localized. In turn it is obvious that the width in \DeltaE depends on the selection in \mes. To illustrate this behavior Fig. \ref{fig:DeltaE_comp_eMC} shows a comparison of truth-matched Monte Carlo data for the electron channel with different \mes selections.
\begin{figure}[h]
  \centering\includegraphics[width=.6\textwidth]{figures/mES_DeltaE_signal/DeltaE_comp}
  \caption{Comparison of the truth-matched \DeltaE distribution for different \mes cut values.}
  \label{fig:DeltaE_comp_eMC}
\end{figure}
To determine the \DeltaE signal region we apply an {\it ad-hoc} \mes cut at $5.26\gevcc$. Since \DeltaE cannot be described by a simple Gaussian function we determine a $2\sigma$ cut by choosing a symmetric cut around $0\gev$ which retains $95.5\%$ of the truth-matched signal events. The resulting cut is 
\begin{equation}
  |\DeltaE| < 1.3 \gev.%more exact 1.37
\end{equation}
Using this \DeltaE cut we determine the \mes cut in a similar way and obtain
\begin{equation}
  \mes > 5.26 \gevcc.
\end{equation}

For the extraction of the signal yield we decide to use $\DeltaE$ which can be fitted more easily than $\mes$.

==> chapters/significance.tex <==
For the significance calculation we repeat the previous fit to data with the signal yields fixed to zero. Since the fit with a signal component already gives a signal yield of zero for the electron channel we can omit this decay mode from the significance calculation.

For the muon case the fit with the signal yield fixed to zero, shown in Fig. \ref{fig:DeltaE_data_noSig}, gives a log-likelihood of $7.52$. 
The fits with the signal component fixed to zero can be found in Figure \ref{fig:DeltaE_data_noSig}.
\begin{figure}[h]
  \begin{center}
    \includegraphics[width=.6\textwidth]{figures/TMVA/cut/muChannel_Fit_OnPeak_DeltaE_noSig}
  \end{center}
  \caption{Fitted \DeltaE distributions in data, with the signal yield fixed to zero for the muon channel.}
  \label{fig:DeltaE_data_noSig}
\end{figure}
The difference in the log-likelihood of $0.10$ translates into a significance of $0.4\sigma$.

==> chapters/strategy.tex <==
STRATEGY STRATEGY STRATEGY

==> chapters/sys_MC_Model.tex <==
For the systematic uncertainty arising from our WI Monte Carlo model we alter the width of the $\LCp \antiproton$ resonance from $100\mevcc$ to $200\mevcc$ and repeat the fits described before. The background descriptions stays unchanged. The newly obtained fit parameters for signal description are given in Tab. 
\begin{figure}[h]
  \begin{center}
    \subfigure[]{
      \includegraphics[width=.48\textwidth]{figures/TMVA/sys/eChannel_DeltaE_sig_bestCut_fit}
      \label{fig:clf_sys_eChannel_fit_sig}
    }
    \subfigure[]{
      \includegraphics[width=.48\textwidth]{figures/TMVA/sys/muChannel_DeltaE_sig_bestCut_fit}
      \label{fig:clf_sys_muChannel_fit_sig}
    }
  \end{center}
  \caption{Fitted signal \DeltaE distribution for the electron \subref{fig:clf_opt_eChannel_fit_sig} and the muon \subref{fig:clf_opt_muChannel_fit_sig} channel. In both cases signal is fitted with the sum of a Cruijff and Gaussian function.}
  \label{fig:sys:sig_cruijff_fit}
\end{figure}
\begin{tabular}{lr}
  \begin{minipage}{.46\textwidth}
    \begin{table}[H]
      \caption{Fit parameter for the \DeltaE fit in signal Monte Carlo for the electron channel.}%FCN = 14.2157542848
      \begin{center}
      \begin{tabular}{lc}
        \toprule
        parameter & value \\\midrule
        $m_{0} $ & $ 0.037 \pm 0.004$\\
        $\sigma_L $ & $ 0.104 \pm 0.004$\\
        $\sigma_R $ & $ 0.530 \pm 0.005$\\
        $\alpha_L$ & $0.058 \pm 0.019$\\
        $\alpha_R$ & $0.017 \pm 0.004$\\
        $\mu$ & $0.040 \pm 0.005$\\
        $\sigma$ & $0.2015 \pm 0.0017$\\
        $f_0$ & $0.764 \pm 0.007$\\
        $N_{\rm sig}$ & $284600 \pm 600$\\
        \bottomrule
      \end{tabular}
      \end{center}
      \label{tab:sys:fitDeltaE_sig_eChannel}
    \end{table}
  \end{minipage} &
  \begin{minipage}{.46\textwidth}
    \begin{table}[H]
      \caption{Fit parameter for the \DeltaE fit in signal Monte Carlo for the muon channel.}
      \begin{center}
        \begin{tabular}{lc}\toprule
          parameter & value \\\midrule
          $m_{0} $ & $ 0.0533 \pm 0.0021$\\
          $\sigma_L $ & $ 0.1247 \pm 0.0016$\\
          $\sigma_R $ & $ 0.301 \pm 0.006$\\
          $\alpha_L$ & $0.076 \pm 0.005$\\
          $\alpha_R$ & $0.128 \pm 0.004$\\
          $\mu$ & $0.663 \pm 0.016$\\
          $\sigma$ & $0.373 \pm 0.006$\\
          $f_0$ & $0.852 \pm 0.009$\\
          $N_{\rm sig}$ & $216200 \pm 500$\\
          \bottomrule
        \end{tabular}
      \end{center}
      \label{tab:sys:fitDeltaE_sig_muChannel}
    \end{table}
  \end{minipage}
\end{tabular}

==> chapters/theory.tex <==
\section{Theory}

This suppression of the two-body decay can be understood in terms of a simple fragmentation model. For the production of a baryon anti-baryon pair an energetic $q\bar{q}$ must be emitted back to back by a gluon, which in turn is highly off mass shell. This decay is suppressed by $\alpha_s/t$, where $t$ is the four-momentum square transferred by the gluon \cite{Suzuki:2007pw}. For the three-body mode the additional meson can carry away much momentum, reducing the momentum transfer of the gluon. A similar picture is described in \cite{Cheng:2001tr} for charmless baryonic \B decays.

For higher multiplicities resonant submodes gain a larger impact, and account for a substantial part of the total branching fraction.
\begin{itemize}
\item for higher modes refer to resonant substructure(?) and increasing number of Feynman graphs
\item impact from external W graph not known -> reachable by semi-leptonic decay
\item previous measurement by BABAR was an inclusive, tagged approach -> reduced statistics
\item subsection on threshold enhancement
\item present THs results w/ and w/o threshold enhancement
\item classify decays according to graphs -> which decays show enhancement, which do not?
\item expectation for semi-leptonic decay
\item comparison with Stephanies analysis ...
\end{itemize}

==> chapters/titleBAD.tex <==
\begin{titlepage}
%\let\footnotesize\small \let\footnoterule\relax
\begin{center}
\begin{flushleft}
       \mbox{\normalsize {\babar\ }Analysis Document \#2553, Version 1}
       \end{flushleft}
       \vskip 15pt
\hbox{}
\vfill
{\huge\bfseries Study of the decay
		\boldmath$\Bm \rightarrow \Lambda_c^+ \antiproton \ellm \nulb$\unboldmath}
\vskip 1cm
University of Rostock\\[2ex]
Torsten Leddig
\vskip 1.5cm
\today
%\date{\today}
%2007, February 05 \\
\end{center}
\vfill
\end{titlepage}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "diplarb"
%%% End: 


==> chapters/vertex_probability.tex <==
Another source for fake signal events, besides wrongly reconstructed $\LCp$ candidates, are random combinations of $\LCp$, $\antiproton$, $\ellm$. To reduce this background we require that all three particles originate from the same vertex, thus reducing combinations of particles originating from the two \B mesons. A comparison of the probability ($P$) for the combined particles to originate from the same vertex can be seen in Fig. \ref{fig:Vtx_Prob}. For the figure the background Monte Carlo sets are scaled to \texttt{OnPeak} data luminosity. The comparison shows a discrepancy between background Monte Carlo and \texttt{OnPeak} data, which is most likely caused by deficits in the simulation of baryonic \B decays for the generic $\BpBm$ and $\BzBzb$ modes. But since a cut in $P(Y)$ does not rely on the overall shape, but on the distribution Monte Carlo gives an adequate model for data. Comparing signal Monte Carlo with the background simulation reveals that background tends to peak near $0$ and diminishs to $0$ for higher $P(Y)$ values, while signal Monte Carlo shows a peak at $0$ as well but stays constant for higher $P(Y)$ values. Based on the experience gained in the analysis of $\Bzb \ra \LCp \antiproton \Km \pip$ \cite{PhysRevD.80.051105,BAD2149} we choose to use
\begin{equation}
  P(Y) > 0.002\;.
\end{equation}
This value should reject a majority of background candidates with tracks originating from both \B mesons, while retaining a large fraction of signal events.
\begin{figure}[h]
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/compareVariables/electron/YcandVtxProb}
    \label{fig:electron:Vtx_Prob}
  }
  \subfigure[]{
    \includegraphics[width=.48\textwidth]{figures/compareVariables/muon/YcandVtxProb}
    \label{fig:muon:Vtx_Prob}
  }
  \caption{Vertex probability for the $\LCp \antiproton \en$ \subref{fig:electron:Vtx_Prob} and $\LCp \antiproton \mun$ \subref{fig:muon:Vtx_Prob} combination. Background Monte Carlo data sets are stacked, \texttt{OnPeak} data and signal Monte Carlo are super-imposed.}
  \label{fig:Vtx_Prob}
\end{figure}
